Towards Faithful Model Explanation in NLP: A Survey

End-to-end neural Natural Language Processing (NLP) models are notoriously difficult to understand. This has given rise to numerous efforts towards model explainability in recent years. One desideratum of model explanation is faithfulness, i.e. an explanation should accurately represent the reasoning process behind the model's prediction. In this survey, we review over 110 model explanation methods in NLP through the lens of faithfulness. We first discuss the definition and evaluation of faithfulness, as well as its significance for explainability. We then introduce recent advances in faithful explanation, grouping existing approaches into five categories: similarity-based methods, analysis of model-internal structures, backpropagation-based methods, counterfactual intervention, and self-explanatory models. For each category, we synthesize its representative studies, strengths, and weaknesses. Finally, we summarize their common virtues and remaining challenges, and reflect on future work directions towards faithful explainability in NLP.

==> fables/figure_attention.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=0.7\textwidth]{imgs/attention.jpeg}
  \caption{An illustration of the self-attention mechanism. Each output vector $y_j$ is a weighted average of affine transformations of all input vectors $X$.}\label{figure:attention}
\end{figure}

==> fables/figure_clark_object.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{imgs/clark_object.png}
  \caption{An attention head in BERT where direct objects attend to their verbs (figure from \citet{clark_what_2019}). The direct objects of interest are highlighted in red.}\label{figure:clark_object}
\end{figure}

==> fables/figure_prop_methods_visual.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=\textwidth]{imgs/deconvnet_guidedbp.jpg}
    \caption{A visualization of DeconvNet and Guided BackPropagation, in comparison with Simple Gradients, on an example cat image (figure adapted from \cite{springenberg_striving_2015}).}
  \label{figure:prop_methods_visual}

\end{figure}



==> fables/figure_sigmoid_tanh.tex <==
\begin{figure}[!tbp]
  \centering
  \subfloat[sigmoid: $y = \frac{1}{1+e^{-x}}$]{
    \includegraphics[width=0.4\textwidth]{imgs/sigmoid.png}
  }
  \hfill
  \subfloat[tanh: $y = \frac{e^{x} - e^{-x}}{e^{x}+e^{-x}}$]{
    \includegraphics[width=0.45\textwidth]{imgs/tanh.png}
  }
\caption{The sigmoid function and the tanh function. Both are ``saturated'' (i.e., the gradient is near-zero) when the input is small or large enough.}\label{figure:sigmoid_tanh}
\end{figure}

==> fables/figure_vig_coref.tex <==
\begin{figure}[!tbp]
  \centering
  \subfloat[Attention from \textit{he}.]{
    \includegraphics[width=0.43\textwidth]{imgs/vig_he.png}
  }
  \hfill
  \subfloat[Attention from \textit{she}.]{
    \includegraphics[width=0.43\textwidth]{imgs/vig_she.png}
  }
\caption{An attention head in GPT-2 that captures coreference (figure from \citet{vig_visualizing_2019}). The left and the right column stand for the output and the input of the attention function, respectively. Darker shades indicate larger attention weights.}\label{figure:vig_coref}
\end{figure}
